Approximate Topological Optimization using Multi-Mode Estimation for Robot Motion Planning

In this extended abstract, we report on ongoing work towards an approximate multimodal optimization algorithm with asymptotic guarantees. Multimodal optimization is the problem of finding all local optimal solutions (modes) to a path optimization problem. This is important to compress path databases, as contingencies for replanning and as source of symbolic representations. Following ideas from Morse theory, we define modes as paths invariant under optimization of a cost functional. We develop a multi-mode estimation algorithm which approximately finds all modes of a given motion optimization problem and asymptotically converges. This is made possible by integrating sparse roadmaps with an existing single-mode optimization algorithm. Initial evaluation results show the multi-mode estimation algorithm as a promising direction to study path spaces from a topological point of view.

==> images/evaluations_figure.tex <==
\begin{figure*}
\centering
 \begin{subfigure}[b]{0.32\textwidth}
      \centering
    \includegraphics[width=\textwidth, height=\textwidth]{images/blender/sphere.png}
     \caption{$S^2$ state space:  twice punctured sphere (4 minima)}
\end{subfigure}
\begin{subfigure}[b]{0.32\textwidth}
      \centering
    \includegraphics[width=0.8\textwidth, height=\textwidth]{images/blender/kleinbottle.png}
     \caption{$K$ state space: punctured Klein bottle state space (3 minima modes).}
\end{subfigure} \begin{subfigure}[b]{0.32\textwidth}
      \centering
    \includegraphics[width=\textwidth, height=\textwidth]{images/blender/torus.png}
     \caption{$T=S^1 \times S^1$ state space: punctured Torus (4 minima)}
\end{subfigure}
\caption{Illustrative toy examples with a point robot on different state spaces. Local optima found after convergence are shown in red. Please note that the minima are relative not only to the cost functional, but also to the optimization method.}
\end{figure*}
